Decentralized Fictitious Play Converges Near a Nash Equilibrium in Near-Potential Games

We investigate convergence of decentralized fictitious play (DFP) in near-potential games, wherein agents preferences can almost be captured by a potential function. In DFP agents keep local estimates of other agents' empirical frequencies, best-respond against these estimates, and receive information over a time-varying communication network. We prove that empirical frequencies of actions generated by DFP converge around a single Nash Equilibrium (NE) assuming that there are only finitely many Nash equilibria, and the difference in utility functions resulting from unilateral deviations is close enough to the difference in the potential function values. This result assures that DFP has the same convergence properties of standard Fictitious play (FP) in near-potential games.

==> Benchmark.tex <==
% !TEX root = Control in state-based anti-coordination network games.tex

%We consider star, line and ring networks, and provide optimal solutions for both static and dynamic MPCAC problems. 

%\begin{figure}[t]
%	\centering
%	\begin{tabular}{cc}
%			\input{figs/star.tex} &
%			\input{figs/line.tex}
%%			\input{figs/ring.tex}
%	\end{tabular}
%\caption{Star and line networks. }
%\label{fig:benchmark_network}
%\end{figure}

\subsection{Star network}

Consider a star network of $n$ players with player 1 in the center. Without loss of generality we assume $s_1 = 1$ and $j \in \ccalS_0$ for $j \notin \{1\}$---see Figure \ref{fig:bipartite}. 

%\begin{proposition} \label{thm_star_staticMPCAC}
%Depending on the utility constants $c_0$ and $c_1$, the optimal solutions to static MPCAC follows. 
%\begin{itemize}
%\item[a)] If $1>c_0$ and $1>c_1 (n-1)$, then $\ccalX = \{1\}$ with $\delta_1 = 0$.
%\item[b)] If $1<c_0$ and $1>c_1 (n-1)$, or $1>c_0$ and $1<c_1 (n-1)$, then $\ccalX = \emptyset$.
%\item[(c)] If $1<c_0$ and $1<c_1 (n-1)$, then $\ccalX = \{1\}$ with either $\delta_1 = 0$ or $1$.
%\end{itemize}
%\end{proposition}
%\begin{myproof}
%In a star network, if $1>c_1 (n-1)$ or $1>c_0$, then the center or the fringe players have all actions strictly dominated by action 1 via \eqref{worst_case_good_response}. If $1<c_0$, then a fringe player eliminates all actions except 0 via \eqref{best_case_bad_response} when the center node takes action 1. If $1<c_1 (n-1)$, then the center player eliminates all actions except 0 via \eqref{best_case_bad_response} when the fringe nodes take action 1. Based on this, in case (a), the algorithm converges to an action profile where all players take action 1. In order to achieve maximum anti-coordination, we select center player to play action 0. In case (b) the algorithm converges in 2 steps to a maximum anti-coordination action profile, i.e., $\{a_1 = 1, a_{-1} = 0\}$ or $\{a_1 = 0, a_{-1} = 1\}$. In case (c), there is no action that is strictly dominated if we do not control a player. Hence, we control center player to take action 0, i.e., $\ccalX=\{1\}$. Then, all fringe players eliminate all actions except action 1. 
%\end{myproof}


%For the dynamic MPCAC, we need to specify the set of nodes controlled at each time step denoted by $\ccalX^t$. We provide optimal policies for dynamic MPCAC problem on a star network. 

\begin{proposition} \label{thm_star_dynamicMPCAC}
The optimal dynamic MPCAC solutions for the star network are as follows. 
\begin{itemize}
\item[(a)] If $1>c_0$ and $1>c_1 (n-1)$, then
\begin{equation}
	\begin{cases}\ccalX^t =\varnothing, \ &\text{if } t < n \\ \ccalX^t =\{1\}, \delta_1^t = 0 &\text{if } t\geq n  \end{cases}
\end{equation}
The resulting optimal cost is $C^* = 1$.
\item[(b)] If $1<c_0$ and $1>c_1 (n-1)$, or $1>c_0$ and $1<c_1 (n-1)$, then $\ccalX^t = \varnothing$ for all $t$.
The resulting optimal cost is $C^* = 0$.
\item[(c)] If $1<c_0$ and $1<c_1 (n-1)$, then $\ccalX^1 = \{1\}$.
\begin{equation}
	\begin{cases}\ccalX^t =\{1\}, \delta_1^t = 0 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
\end{equation}
The resulting optimal cost is $C^* = 2/n$.
%
%\item If $1>c_1 (n-1)$ and $1<c_0$, or  $1<c_1 (n-1)$ and $1>c_0$, then $|\ccalC| = 0$.
%\item If $1>c_1 (n-1)$ and $1>c_0$, then $\ccalC_t = \{1\}$ for all $t=1,2,\dots$.
%\item If $1<c_1 (n-1)$ and $1<c_0$, then $\ccalC_0 = \{1\}$.
\end{itemize}
\end{proposition}
\begin{myproof}
In cases (a) and (b), the game is dominance solvable. Further, the algorithm converges in $t\leq 2$ steps. Lemma \ref{thm_dominance_solvable} together with Theorem \ref{thm_vertex_cover} gives the optimal policies (a) and (b), respectively. 
In case (c), the game is not dominance solvable and there exists two Nash equilibria belonging to $M(\ccalG_B)$: $(a_1=0,\{a_i=1\}_{i\neq 1})$ and $(a_1 = 1, \{a_i=0\}_{i\neq 1})$. By Lemma \ref{thm_anti_coordination_equilibria}, the optimal policy will induce the dynamics to converge to one of these configurations. Either of these equilibria can be achieved through a dynamic policy that targets only the center node for two time steps, which gives the optimal cost $2/n$. For instance, we set $\delta_1^0= 0$  so that fringe players select $a_i^1=1$.  We continue with $\delta_1^1 = 0$, so that the center node's unforced action is 0 by \eqref{best_case_bad_response}. We lift the control for all $t\geq 2$, by which time the players are in equilibrium and MAC is achieved. This policy is optimal because there cannot be a policy that achieves a smaller objective value than $2/ n$ and achieve MAC.
\end{myproof}

The above analysis exemplifies the three uncontrolled action profiles \eqref{eq_action_profile_k} that can arise in a star network: (a) all players decide but MAC is not satisfied; (b) MAC is satisfied; (c)  all players remain undecided. In case (a), we control center player to induce MAC. In case (b), no control is necessary. In case (c), we control the center player to trigger decisions for the fringe players. 


%The optimal action profile and its proof are similar to the static case. There are two significant differences between the dynamic and static problem. If the algorithm converges to an action profile in which some neighboring pairs of players end up taking action 1, e.g., case (a), then we have to anti-coordinate the corresponding links by controlling one of the players at the end of the time horizon $n$. If the algorithm is going to converge to an action profile where we will have undecided neighboring players (case (c)), we can make these players anti-coordinate by initially controlling one of the neighbors temporarily for two time steps. In case (a), we incur a cost of 1 because if we lift our control of the center player, it will always revert back to $a_1=1$. In contrast, in case (c), we only need to control the player $1$ for two steps, because it will not revert to $a_1 = 1$ by the time its neighbors are taking action 1. 

\subsection{Line network}

 We consider a line network in which the neighborhood of player $i\in\ccalN \setminus \{1,n\}$ is given by $\ccalN_i=\{i-1,i+1\}$. The players at the endpoints have neighbor sets $\ccalN_1 = \{2\}, \ccalN_n = \{n-1\}$.  The type configuration alternates between types 0 and 1: $i \in \ccalS_0$ for $i$ odd, and $i\in\ccalS_1$ for $i$ even. We will also refer to the subsets $\ccalS_m^{\text{odd}}, \ccalS_m^{\text{even}}$ for $m\in\{0,1\}$ to denote every odd (even) player from the set $\ccalS_m$ along the line. In the following, we consider all possible payoff cases for the line network.
 
% six payoff constant cases that ensure an exhaustive analysis for the line network.%. We consider an odd number of players on the line network.

%We consider a line network in which the neighborhood of player $i\in\ccalN_i \setminus \{1,n\}$ is given by $i-1$ and $i+1$, i.e., $\ccalN_i=\{i-1,i+1\}$. The players at the end of the line network $i=1$ and $i=n$ are connected to the players after ($i=2$) and before ($i=n-1$), respectively.  The state configuration alternates between states 0 and 1: $i \in \ccalS_0$ for $i$ odd, and $i\in\ccalS_1$ for $i$ even -- see Figure \ref{fig:benchmark_network}. We also use the index notation $\{i_1,i_2,\ldots,i_{\lceil n/2 \rceil} \} := \{1,3,5,\ldots,n \ \text{or } n-1\}$ to be the indices of $\ccalS_0$ players, and $\{j_1,j_2,\ldots,j_{\lfloor n/2 \rfloor} \} := \{2,4,6,\ldots,n \ \text{or } n-1\}$ to be the indices of $\ccalS_1$ players. Also, let $\ccalS_0^{\text{odd}} := \{i_k : k \ \text{is odd}\}$ and $\ccalS_1^{\text{odd}} := \{j_k : k \ \text{is odd}\}$. In the following analysis, we consider six payoff constant cases that ensure an exhaustive analysis for the line, and in the next section, the ring network.

%\begin{figure}
%	\includegraphics[scale=.75]{figs/c0c1_regions.pdf}
%	\caption{The payoff constant cases studied in line and ring networks, labeled (a)-(f). The cases not studied in the analysis either admit the same optimal solution or a symmetric solution where player states are flipped, due to the symmetry of the payoff constants. For example, the lower right case is dominance solvable in the same manner as (c), but the players that take action 1 are the opposite state and vice versa.}
%	\label{parameter_space}
%\end{figure}


%%
%\begin{proposition}\label{static_odd_line}
%	Depending on the utility constants $c_0$ and $c_1$, the optimal control set for the static MPCAC problem for a line network with $n$ odd  is
%	\begin{itemize}
%		\item[a)] If $1 > 2c_0$ and $1 > 2c_1$, then $\ccalX = \ccalS_1$, $|\ccalX| = \lfloor n/2 \rfloor$, and $\delta_{\ccalS_1} = 0$.
%		\item[b)] If $1 > 2c_0$ and $2c_1 > 1 > c_1$, then $\ccalX = \varnothing$.
%		\item[c)] If $1 > 2c_0$ and $c_1 > 1$, then $\ccalX = \varnothing$.
%		\item[d)] If $2c_0 > 1 > c_0$ and $2c_1 > 1 > c_1$, then $\ccalX = \ccalS_1^{\text{even}}, \{\delta_i\}_{i\in\ccalX} = 0$, and $|\ccalX| = \lfloor n/4 \rfloor$.
%		\item[e)] If $c_0 > 1$ and $2c_1 > 1 > c_1$, then $|\ccalX| = 1$ where $\ccalX$ is any one player $i$, with $\delta_i = 0$ ($1$) if $i\in\ccalS_0$ ($\ccalS_1$).
%		\item[f)] If $c_0 > 1$ and $c_1 > 1$, then $|\ccalX| = \lceil (n-1)/4 \rceil$, where  $\ccalX =  \ccalS_0^{\text{even}}$, with $\delta_{\ccalX} = 1$.
%	\end{itemize}
%\end{proposition}
%\begin{myproof}
%	\begin{itemize}
%		\item[a)] The game is dominance solvable with the unique Nash equilibrium $a_i = 1$ for all $i\in\ccalN$. The minimum vertex cover is $\ccalX =\ccalS_1$, and forcing action 0 induces the solution.
%		\item[b)] The game is dominance solvable with the unique Nash equilibrium $a_{\ccalS_0} = 1$, $a_{\ccalS_1} = 0$.
%		\item[c)] Same proof as (b).
%		\item[d)] Consider controlling $\ccalS_1$ players spaced three nodes apart along the line with action 0. These consist of the even-indexed $\ccalS_1$ players. In two time steps, the nodes in between will converge to the equilibrium action inducing maximum anti-coordination. The smallest number of nodes to control in this manner is $ \lfloor n/4 \rfloor$. Sparser placement of control results in undecided players.
%		\item[e)] If $\ccalX$ selects a single $i \in \ccalS_1$ to play $a_i=1$, its $\ccalS_0$ neighbors decide on action 0 ($1 < c_0$). At the next iteration, the next $\ccalS_1$ players will decide on action 1 ($1 > c_1$). This cascades down the entire line, resulting in maximum anti-coordination. The same holds if $\ccalX$ selected a single $i \in\ccalS_0$  to play $a_i = 0$.
%		\item[f)] In a similar manner as case (d), $\ccalX$ can be chosen to be every other $\ccalS_0$ player along the line network, forcing with action 1 to cause two-hop cascades along the network in two time steps.
%	\end{itemize}
%\end{myproof}
%\begin{myproof}
%	\begin{itemize}
%		\item[a)] The game is dominance solvable and all nodes decide on action 1 after one iteration. Since $|\ccalS_1| = (n-1)/2 < |\ccalS_0| = 1 + (n-1)/2$, the minimum vertex cover is chosen as $\ccalX =\ccalS_1$.
%		\item[b)] The game is dominance solvable with the unique Nash equilibrium $(a_{\ccalS_0} = 1$, $a_{\ccalS_1} = 0)$ achieving maximum anti-coordination.
%		\item[c)] Same proof as (b).
%		\item[d)] Consider controlling $\ccalS_1$ players spaced three nodes apart along the line with action 0. These consist of the even-indexed $\ccalS_1$ players. In two time steps, the nodes in between will converge to the equilibrium action inducing maximum anti-coordination. The smallest number of nodes to control in this manner is $ \lfloor n/4 \rfloor$. Sparser placement of control will result in players remaining undecided.
%		\item[e)] In this case, the dynamics produces no decided players. If $\ccalX$ selects a single state-1 player to play action 1, its neighbors decide on action 0 ($1 < c_0$). At the next iteration of the algorithm, the next state-1 players will decide on action 1 ($1 > c_1$). This cascades down the entire line, resulting in maximum anti-coordination. The same holds if $\ccalX$ selected a single state-0 player to play action 0.
%		\item[f)] The proof is similar to Proposition \ref{even_line_proposition}. Here, since node $n$ is a state-0 node, $\ccalX$ can simply be chosen to be every other state-0 node along the line network, forcing them to play action 1.
%	\end{itemize}
%\end{myproof}

%
\begin{proposition}\label{dynamic_odd_line}
	Depending on the utility constants $c_0$ and $c_1$, the optimal control policy $(\{\ccalX^t\},\Delta)$ for the dynamic MPCAC problem on a line network with $n$ odd  is
	\begin{itemize}
		\item[a)] If $1 > 2c_0$ and $1 > 2c_1$, then 
		\begin{equation}
			\begin{cases}\ccalX^t =\varnothing \ &\text{if } t <n \\ \ccalX^t =\ccalS_1, \{\delta_i^t\}_{i\in \ccalS} = 0 &\text{if } t \geq n  \end{cases}
		\end{equation}
		which gives the optimal cost $C^* =  \lfloor n/2 \rfloor$.
		\item[b)] If $1 > 2c_0$ and $2c_1 > 1 > c_1$, then $\ccalX^t = \varnothing$ for all $t \geq 0$.
		\item[c)] If $1 > 2c_0$ and $c_1 > 1$, then $\ccalX^t = \varnothing$ for all $t \geq 0$.
		\item[d)] If $2c_0 > 1 > c_0$ and $2c_1 > 1 > c_1$, then
		\begin{equation}
			\begin{cases}\ccalX^t = \ccalS_1^{\text{even}}, \delta_{\ccalX^t}^t = 0 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
		\end{equation}
		which gives the optimal cost $C^* =  2\lfloor n/4 \rfloor/n$.
		\item[e)] If $c_0 > 1$ and $2c_1 > 1 > c_1$, then
		\begin{equation}
			\begin{cases}\ccalX^t = \{i\}, \delta_i^t = s_i \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
		\end{equation}
		for any $i \in \ccalN$. This gives the optimal cost $C^* =  2/n$.
%If $c_0 > 1$ and $2c_1 > 1 > c_1$, then $|\ccalX^t| = 1$ for $t=0,1$ and $\ccalX^t = \varnothing$ for $t\geq 1$. Here $\ccalX_1 = \ccalX_2$ can be chosen as any one player. If the player is state-0, it forces it to play action 0. If the player is state-1, it forces it to play action 1.
		\item[f)] Suppose $c_0 > 1$ and $c_1 > 1$.  Then 
		\begin{equation}
			\begin{cases}\ccalX^t = \ccalS_0^{\text{even}}, \delta_{\ccalX^t}^t = 1 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
		\end{equation}
		 gives the optimal cost $C^* =  2\lceil (n-1)/4 \rceil/n$.
	\end{itemize}
\end{proposition}
%\begin{myproof}
%	\begin{itemize}
%		\item[a)] The game is dominance solvable, and converges at $t=1$ to $a = (1,\ldots,1)$. By Corollary \ref{thm_optimal_vertex_cover}, the optimal policy is the vertex cover solution.
%		\item[b)]  The game is dominance solvable, and converges at $t=2$ to the unique Nash equilibrium $a$ s.t. $a_i = 1 \ \forall i\in\ccalS_0$ and $a_i = 0 \ \forall i\in\ccalS_1$, achieving maximum anti-coordination.  Lemma \ref{thm_dominance_solvable} asserts the optimal policy is the empty set.
%		\item[c)] Same proof as (b).
%		\item[d)] The action profile $a_{\ccalS_0} = 1$, $a_{\ccalS_1} = 0$ is the only Nash equilibrium achieving maximum anti-coordination. By Lemma \ref{thm_anti_coordination_equilibria}, the optimal policy induces convergence to this equilibrium by $t=n$. Only the endpoint players $\{1,n\}\in\ccalS_0$ have action 1 as a dominant strategy $(1 > c_0)$, and all other players will remain undecided in the absence of control. Hence, the policy that gives convergence to $a$ with minimal cost selects every even $\ccalS_1$ players to play 0 for two time steps, given in the Proposition statement d).
%		\item[e)] The game is not dominance solvable, but there are two Nash equilibria $a^*$, $\hat a$ giving maximum anti-coordination, where $(a_{\ccalS_0}^* = 0$, $a_{\ccalS_1}^* = 1)$ and $(\hat{a}_{\ccalS_0} = 1$, $\hat{a}_{\ccalS_1} = 0)$. By Lemma \ref{thm_anti_coordination_equilibria}, the optimal policy induces convergence to one of these equilibria by $t=n$. One can check that a dynamic policy incurring total cost $2/n$ (controlling a single node for two time-steps) induces convergence to $a^*$, and any dynamic policy inducing convergence to $\hat a$ has cost strictly greater than $2/n$ because a player in $i\in\ccalS_1$ needs $a_{i-1}^{t-1} = a_{i+1}^{t-1} = 1$ in order to play the equilibrium action $a_i^t = 0$ (due to $1<2c_1$). Such a convergence would require controlling more than a single node for two time steps.
%		\item[f)] One of the two Nash equilibria $a^*$, $\hat a$ are selected by Lemma \ref{thm_anti_coordination_equilibria}. Selecting $\hat a$ gives the minimal cost when every odd $\ccalS_0$ player is controlled with action 1 for two time-steps, which causes the players in between these selections to decide on the equilibrium actions. Similarly, selecting $a^*$ also gives the minimal cost when every odd $\ccalS_1$ player, including the last one, is controlled with action 1 for two time-steps.
%	\end{itemize}
%\end{myproof}
%
%When considering even number of players $n$ in the line network, we obtain similar results. For brevity, we present the results but omit the proofs because they follow similar arguments as Proposition \ref{dynamic_odd_line}. Here, the type configuration in the network also alternates s.t. $i \in \ccalS_0$ if $i$ is odd, and $s_i \in \ccalS_1$ if $i$ is even.
%
%%\begin{myproof}
%%	The proofs of dynamic MPCAC follow similar arguments from Proposition \ref{static_odd_line} in the choice of control sets $\ccalX^t$. In the dynamic MPCAC formulation however, it is not always required to fix the selected players in the desired control action for all times (cases d,e, and f). In these cases, the control player will consolidate its action after two time steps. In case a), the control players will never consolidate their actions  and hence control is necessary for all times $t \geq 0$.
%%\end{myproof}
%
%\begin{proposition}\label{even_line_static}
%	Depending on the utility constants $c_0$ and $c_1$, the optimal solutions to static MPCAC for a line network with $n$ even is
%	\begin{itemize}
%		\item[a)] If $1 > 2c_0$ and $1 > 2c_1$, then $\ccalX = \ccalS_0$ or $\ccalS_1$ with $\delta_{\ccalX} = 0$. Then, $|\ccalX| = n/2$.
%		\item[b)] If $1 > 2c_0$ and $2c_1 > 1 > c_1$, then $\ccalX = \{n\}$ with $\delta_n = 0$.
%		\item[c)] If $1 > 2c_0$ and $c_1 > 1$, then $\ccalX = \varnothing$. 
%		\item[d)] If $2c_0 > 1 > c_0$ and $2c_1 > 1 > c_1$, then $\ccalX = \ccalS_1^{\text{odd}}$ with $\delta_{\ccalX} = 0$. Then $|\ccalX| = \lceil n/4 \rceil$.
%		\item[e)] If $c_0 > 1$ and $2c_1 > 1 > c_1$, then $\ccalX = \varnothing$. 
%		\item[f)] If $c_0 > 1$ and $c_1 > 1$, then $\ccalX = \ccalS_1^{\text{odd}}$ with $\delta_{\ccalX} = 1$. Then $|\ccalX| = \lceil n/4 \rceil$.
%	\end{itemize}
%\end{proposition}
%%\begin{myproof}
%%	\begin{itemize}
%%		\item[a)] All nodes will play $a_i=1$ after a single iteration of Algorithm \ref{local_alg} . Hence, the only way to ensure anti-coordination is to select $\ccalX = \{i : s_i = 0 \}$ or $\{i : s_i = 1\}$ and force these nodes to play $a_i = 0$.
%%		\item[b)] All nodes with $s_i = 0$ will play $a_i = 1$ after one iteration of the algorithm. The $n/2 - 1$ nodes  that are sandwiched between such nodes then will play $a_i = 0$, and node $n$ decides to play $a_i = 1$ in the next iteration. However, we do not have maximum anti-coordination since $a_n = a_{n-1} = 1$. Hence, setting $\ccalX = \{n\}$ solves the problem.
%%		\item[c)] All nodes with $s_i = 0$ will play $a_i = 1$, while all nodes with $s_i = 1$ remain undecided after one iteration. In the next iteration, all nodes $s_i=1$ then decide on $a_i = 0$. Hence, no control is required.
%%		\item[d)] Without control, the algorithm converges in a single iteration to $(a_1,\{a_j\}_{j=2}^{n-1},a_n) = (1, \{\epsilon\}_{j=2}^{n-1},1)$. A middle node with $s_i = 0$ needs both neighbors playing $a_j = 0$ to decide on $a_i = 1$. Hence, setting $\ccalX = \{i : s_i = 1\}$ to force actions to zero results in all middle state-zero nodes to play 1, and the endpoint $a_n = 0$ to give anti-coordination.
%%		\item[e)] The algorithm converges in $n$ iterations to maximum anti-coordination with $(a_1,\ldots,a_n) = (0,1,\ldots,0,1)$. The decision-making starts at $a_n = 1$ after the first iteration (all others $\{a_j\}_{j < n}$ undecided), $a_{n-1} = 0$ after the second ($\{a_j\}_{j < n-1}$ undecided), and so on. Hence, no control is necessary.
%%		\item[f)] Without control, the algorithm does not result in any decisions made. A state-1 node (resp. a state-0 node) needs one neighbor playing action 1 to decide on action 0. Also, a state-0 node decides on action 1 if both its neighbors are playing action 0. Maximum anti-coordination can be achieved by forcing $a_1 = 1$, and subsequently every other state-0 to play action one. This partitions the line into strings (not including controlled nodes) with state configuration $(1,0,1)$, where after two iterations will converge to the action $(0,1,0)$. The three nodes at the end, $\{n-2,n-1,n\}$ then can be decided by controlling $\{n-1\}$ to play $a_{n-1} = 1$.
%%	\end{itemize}
%%\end{myproof}
%
%
%\begin{proposition}\label{even_line_dynamic}
%	Depending on the utility constants $c_0$ and $c_1$, the optimal solutions to the dynamic MPCAC problem for a line network with $n$ even is
%	\begin{itemize}
%		\item[a)] If $1 > 2c_0$ and $1 > 2c_1$, then 
%		\begin{equation}
%			\begin{cases}\ccalX^t =\varnothing \ &\text{if } t <n \\ \ccalX^t = \ccalS_0 \ \text{or } \ccalS_1, \{\delta_i^t\}_{i\in \ccalS} = 0 &\text{if } t \geq n  \end{cases}
%		\end{equation}
%		which gives the optimal cost $C^* =   n/2 $.
%		\item[b)] If $1 > 2c_0$ and $2c_1 > 1 > c_1$, then
%		\begin{equation}
%			\begin{cases}\ccalX^t =\varnothing \ &\text{if } t <n \\ \ccalX^t = \{n\}, \delta_n^t = 0 &\text{if } t \geq n  \end{cases}
%		\end{equation}
%		which gives the optimal cost $C^* =   1 $.
%		\item[c)] If $1 > 2c_0$ and $c_1 > 1$, then $\ccalX^t = \varnothing$ for all $t \geq 0$.
%		\item[d)] If $2c_0 > 1 > c_0$ and $2c_1 > 1 > c_1$, then
%		\begin{equation}
%			\begin{cases}\ccalX^t =\ccalS_1^{\text{odd}} \cup \{n\}, \delta_{\ccalX^t}^t = 0 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
%		\end{equation}
%		which gives the optimal cost $C^* = 2\lceil n/4 \rceil/n$.
%		\item[e)] If $c_0 > 1$ and $2c_1 > 1 > c_1$, then
%		\begin{equation}
%			\begin{cases}\ccalX^t = \{i\}, \delta_i^t = s_i \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
%		\end{equation}
%		for any $i \in \ccalN$. This gives the optimal cost $C^* =  2/n$.
%%If $c_0 > 1$ and $2c_1 > 1 > c_1$, then $|\ccalX^t| = 1$ for $t=0,1$ and $\ccalX^t = \varnothing$ for $t\geq 1$. Here $\ccalX_1 = \ccalX_2$ can be chosen as any one player. If the player is state-0, it forces it to play action 0. If the player is state-1, it forces it to play action 1.
%		\item[f)] Suppose $c_0 > 1$ and $c_1 > 1$. Then
%		\begin{equation}
%			\begin{cases}\ccalX^t = \ccalS_1^{\text{odd}}, \delta_{\ccalX^t}^t = 1 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
%		\end{equation}
%		 gives the optimal cost $C^* =  2\lceil n/4 \rceil/n$.
%	\end{itemize}
%\end{proposition}

%\subsection{Ring network}
%Here, we consider a ring network with alternating type configuration and where $n$ is even. For convention, we index the players in the same fashion as the line network above, and alternate types between $\ccalS_0, \ccalS_1$ - i.e., odd (even) indices are $\ccalS_0$ ($\ccalS_1$) players.
%%
%\begin{proposition}\label{static_even_ring}
%	Depending on the utility constants $c_0$ and $c_1$, the optimal solutions to static MPCAC for a ring  network with $n$ even  is
%	\begin{itemize}
%		\item[a)] If $1 > 2c_0$ and $1 > 2c_1$, $\ccalX = \ccalS_0$ or $\ccalS_1$, and $|\ccalX| = n/2$.
%		\item[b)] If $1 > 2c_0$ and $2c_1 > 1 > c_1$, $\ccalX = \varnothing$.
%		\item[c)] If $1 > 2c_0$ and $c_1 > 1$, $\ccalX = \varnothing$.
%		\item[d)] If $2c_0 > 1 > c_0$ and $2c_1 > 1 > c_1$,  $\ccalX = \ccalS_0^{\text{odd}}$ or $\ccalS_1^{\text{odd}}$ with $\delta_{\ccalX} = 1$. Then, $|\ccalX| = \lceil n/4 \rceil$.
%		\item[e)] If $c_0 > 1$ and $2c_1 > 1 > c_1$,  $\ccalX = \{i\}$ with $\delta_i = s_i$ for any $i\in\ccalN$. Then  $|\ccalX| = 1$. 
%		\item[f)] If $c_0 > 1$ and $c_1 > 1$,  either $\ccalX =\ccalS_0^{\text{odd}}$ or $\ccalX =\ccalS_1^{\text{odd}}$ with $\delta_{\ccalX} = 1$. Then $|\ccalX| = \lceil n/4 \rceil$.
%	\end{itemize}
%\end{proposition}
%\begin{myproof}
%	\begin{itemize}
%		\item[a)] The game is dominance solvable with all nodes playing action 1. Hence, influence of either all type-0 or type-1 nodes gives the solution.
%		\item[b)] The game is dominance solvable, which converges to maximum anti-coordination (type-0 playing 1, type-1 playing 0) without influencing any nodes.
%		\item[c)] Same argument as (b).
%		\item[d)] The learning algorithm produces no decided nodes. Controlling a single node to play 0 results in the algorithm converging in the next iteration, with its two neighbors playing 1. Hence, by controlling every other node of one type (every 4 along the ring) to play 0, the algorithm will converge to maximum anti-coordination in two iterations.
%		\item[e)] The algorithm produces no decided nodes. If a single type-0 node is forced to play 0, decisions will be cascaded along the ring resulting in maximum anti-coordination. Similarly, one could influence a single type-1 node to play 1.
%		\item[f)] Same argument as (d).
%	\end{itemize}
%\end{myproof}
%%
%\begin{proposition}\label{dynamic_even_ring}
%	Depending on the utility constants $c_0$ and $c_1$, the optimal solutions to dynamic MPCAC for a ring  network with $n$ even  is
%	\begin{itemize}
%		\item[a)] If $1 > 2c_0$ and $1 > 2c_1$
%		\begin{equation}
%			\begin{cases}\ccalX^t =\varnothing \ &\text{if } t <n \\ \ccalX^t = \ccalS_0 \ \text{or } \ccalS_1, \{\delta_i^t\}_{i\in \ccalS} = 0 &\text{if } t \geq n  \end{cases}
%		\end{equation}
%		The resulting optimal cost is $C^* = n/2$.
%		\item[b)] If $1 > 2c_0$ and $2c_1 > 1 > c_1$, $\ccalX^t = \varnothing$ for all $t\geq 0$.
%		\item[c)] If $1 > 2c_0$ and $c_1 > 1$, $\ccalX^t = \varnothing$ for all $t\geq 0$.
%		\item[d)] If $2c_0 > 1 > c_0$ and $2c_1 > 1 > c_1$,
%		\begin{equation}
%			\begin{cases}\ccalX^t = \ccalS_1^{\text{odd}}, \delta_{\ccalX^t}^t = 1 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
%		\end{equation}
%		The resulting optimal cost is $C^* =  2\lceil n/4 \rceil/n$.
%		\item[e)] If $c_0 > 1$ and $2c_1 > 1 > c_1$,
%		\begin{equation}
%			\begin{cases}\ccalX^t = \{i \}, \delta_{i}^t = s_i \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
%		\end{equation}
%		The resulting optimal cost is $C^* = 2/n$.
%		\item[f)] If $c_0 > 1$ and $c_1 > 1$, then either
%		\begin{equation}
%			\begin{cases}\ccalX^t = \ccalS_0^{\text{odd}}, \delta_{\ccalX^t}^t = 1 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
%		\end{equation}
%		or
%		\begin{equation}
%			\begin{cases}\ccalX^t = \ccalS_1^{\text{odd}} , \delta_{\ccalX^t}^t = 1 \ &\text{if } t =0,1 \\ \ccalX^t =\varnothing &\text{if } t > 1  \end{cases}
%		\end{equation}
%		 gives the optimal cost $C^* =  2\lceil n/4 \rceil/n$.
%	\end{itemize}
%\end{proposition}
%\begin{myproof}
%	We omit the details of the proof for brevity. The proof utilizes similar arguments from Proposition \ref{dynamic_odd_line} by invoking Lemmas \ref{thm_dominance_solvable}, \ref{thm_anti_coordination_equilibria}, and  \ref{thm_vertex_cover}, as well as the structural arguments from the proof of Proposition \ref{static_even_ring}.
%\end{myproof}
%\begin{myproof}
%	The proofs of dynamic MPCAC follow similar arguments from Proposition \ref{static_even_ring} in the choice of control sets $\ccalX^t$. In the dynamic MPCAC formulation however, it is not always required to fix the selected players in the desired control action for all times (cases d,e, and f). In these cases, the control player will consolidate its action after two time steps. In case a), the control players will never consolidate their actions  and hence control is necessary for all times $t \geq 0$.
%\end{myproof}
%\subsection{Discussion}
\noindent The optimal control policies vary depending on the payoff constants. If all players decide to play action 1 as a result of the learning process, then we solve a minimum vertex covering problem along the lines of Theorem \ref{thm_vertex_cover}, and the players selected have to be controlled for all times $t\geq n$---case (a) in all of the propositions in this section. If the game is dominance solvable and all links are inactive in the equilibrium action profile, the optimal policy is the empty set---see \ref{thm_star_dynamicMPCAC}(b),  \ref{dynamic_odd_line}(b,c). If a subset of players remain undecided as a result of the learning algorithm and all links between decided players are inactive, an optimal policy can be found by leveraging Lemma \ref{thm_anti_coordination_equilibria}. In the benchmark examples, these policies required controlling a subset of the players for two time steps, causing the undecided players in the other type to decide in the first step and the controlled players to consolidate their decisions in the second time step. %We only need this subset to be controlled for two time steps. The neighboring players will decide on actions after the first time step, and the controlled players use their neighbors' decisions to consolidate their (unforced) actions in the second time step. Thus, the control can be lifted and no player will revert from their decided actions. The resultant action profile is a Nash equilibrium action profile that satisfies maximum anti-coordination. Hence, there is no need to make control efforts after time $n$. 
Consequently, we can control a smaller subset of players and leverage the learning dynamics to create cascades of decision-making---see cases (d-f) in Propositions \ref{dynamic_odd_line}. In the latter scenarios, the policy suggested by Theorem \ref{thm_vertex_cover} is an upper bound of the optimal policy. The optimal static policies are similar to the dynamic MPCAC policies presented here.

==> conclusion.tex <==
% !TEX root = Control in state-based anti-coordination network games.tex

We considered the control of players' learning processes in a population to influence the emergent outcome in the context of anti-coordination network games. With the goal to promote maximum anti-coordination with minimum effort, we developed computationally tractable methods that determine when to control which players, and how to control them. An algorithm that sequentially selected players according to their influence in promoting anti-coordination in the future performed well in random networks with arbitrary population sizes.

%In this paper, we studied state-based anti-coordination network games where the players follow distributed learning dynamics. We formulated an optimal control problem for finding the minimum number of players to control that ensure the dynamics converge to maximum possible disagreement. We characterized the optimal policies for a line network for a range of payoff parameters, and find in some cases, cascades of decision-making can be leveraged to minimize control effort. For general networks, we proposed a greedy algorithm that computes a feasible, though often suboptimal, control policy to the problem, and evaluated its effectiveness on random bipartite networks through numerical simulations.


%Developing algorithms that achieve optimal behavior while conforming with the computational and informational limitations of the players is of interest given the ubiquity of noncooperative interactions that arise among actors in networked systems, e.g., energy, communication \cite{Bacci_et_al_2016} or autonomous systems \cite{marden2009cooperative}. Game theoretic learning algorithms are tractable decentralized models for decision-making in networked systems. These algorithms while accounting for local information access \cite{Swenson_et_al_2014} and coupled action spaces \cite{yi2017distributed} restrict attention to particular classes of games, e.g., aggregative \cite{parise2015network}, potential \cite{swenson2018distributed}, convex \cite{scutari2010convex}, to guarantee convergence to individually optimal behavior, i.e., a Nash equilibrium action profile. 
%
%A Nash equilibrium is optimal from the perspective of players. However, it can be inefficient and undesired at the system level. A canonical example of this is the tragedy of the commons which describes the phenomenon in which selfish learning behavior leads to the worst possible outcome for the entire population \cite{hardin1968tragedy}. Given the possibility of emergence of undesired outcomes, it is of interest to characterize the inefficiency of Nash equilibria \cite{marden2014generalized}, design payoffs prior to start of the game \cite{Li_Marden}, or develop incentive mechanisms given predetermined payoffs \cite{riehl2018incentive} in order to achieve system-wide desired outcomes. 
%
%In this paper, we consider an incentive mechanism with the goal to induce anti-coordination among players in a state-based network anti-coordination game by controlling a small number of players. In a state-based network anti-coordination game, players belong to one of two possible states. We assume there is a preferred selfish action, e.g., defecting in prisoners' dilemma, in the absence of any neighboring players. A player's payoff decreases as more of its neighbors belonging to the opposite state take the preferred action (Section \ref{sec:model}). These games can be used to model individual behavior during the spread of an epidemic in a population where the states are healthy and sick individuals, the actions represent the level of precautionary measures taken, and payoffs capture the risk of disease transmission to healthy from sick individuals \cite{eksin2017disease}. In these games two neighboring players anti-coordinate when at least one of the players do not take the selfish action, e.g., not taking  precautionary measures during an epidemic.
%
%We formulate the minimum player control for anti-coordination problem as a mixed integer program where the decision variables include which players to control, and how to control them (Section \ref{sec:MPCAC}). We assume players follow learning dynamics based on a decentralized algorithm that mimics the process of iterated elimination of strictly dominated actions in the absence of any control \cite{Fudenberg_Levine_1998}. We find a feasible policy that upper bounds the optimal policy by solving a minimum cardinality vertex covering problem on a reduced bipartite network (Theorem \ref{thm_vertex_cover}). In general, this policy is not optimal if there exists a way to cause cascades of anti-coordination among multi-hop neighbors via the learning dynamics by only controlling a few players. We characterize the optimal policy on a line network of arbitrary size for every possible payoff constant (Section \ref{sec:benchmark_optimal}). The optimal policy exhibits use of cascades to achieve anti-coordination. We also propose a greedy algorithm that finds a feasible, though often suboptimal, solution by sequentially disconnecting the player with the most active links in the network. We assess the algorithm in numerical experiments on random bipartite networks (Section \ref{sec:greedy}).

==> results_learning_dynamics.tex <==
% !TEX root = Control in state-based anti-coordination network games.tex

\subsection{Game theoretic preliminaries}
We consider the  Nash equilibrium solution concept as a rational action profile. A Nash equilibrium (NE) $a^{\text{NE}} \in [0,1]^n$ is an action profile that satisfies
%
\begin{align} \label{Nash_definition}
u_i(a_i^{\text{NE}}, a_{\ccalN_i}^{\text{\text{NE}}}) \geq  u_i(a_i, a_{\ccalN_i}^{\text{NE}}) \quad a_i \in [0,1], i \in \ccalN
\end{align}
%
% where $a_{\ccalN_i}^{\text{NE}} := \{a_{j}^{\text{NE}}: j\in \ccalN_i \}$.
%
In other words, the individuals best-respond to the NE actions of other individuals. For a given neighbor action profile $a_{\ccalN_i}$ the best response for player $i$ is
%
\begin{align}
BR_i(a_{\ccalN_i}) &:= \argmax_{a_i \in [0,1]} u_i(a_i, a_{\ccalN_i}) \label{best_response} \\
& = \bbone\left({1} >  (c_0 (1-s_i)+c_1 s_i) \sum_{j\in \ccalN_i} a_j \right) \label{best_response_specific}
\end{align}
%
where $\bbone(\cdot)$ is an indicator function. Since the payoffs are linear in self-actions, the actions that maximize the payoffs are in the extremes---$a_i =1$ or $a_i = 0$---depending on the types and actions of their neighbors. 
We can equivalently represent the NE definition in \eqref{Nash_definition} by using the best response definition,  
%
\begin{align} \label{NE_best_response}
a_i^{\text{NE}} = BR_i(a_{\ccalN_i}^{\text{NE}}) \quad \forall i\in \ccalN.
\end{align}
%

The notion of strictly dominated is defined in the following.

%
\begin{definition}[Strictly dominated action] \label{strictly_dominated_definition}
An action $a_i \in [0,1]$ is strictly dominated if and only if there exists an action $a_i' \in [0,1]$ such that 
\begin{equation}\label{eq:strictly_dominated_definition}
u_i(a_i', a_{\ccalN_i}) >  u_i(a_i, a_{\ccalN_i}) \quad \forall a_{\ccalN_i}\in \ccalA_{\ccalN_i}.
\end{equation}
\end{definition}
%
If an action $a_i$ is strictly dominated then there exists a more preferable action $a_i'$ for any circumstance. From \eqref{NE_best_response}, a strictly dominated action cannot be rational .
%
%\red{The algorithm is based on the iterated elimination process in which the dominated actions are eliminated in a sequential manner. }
%\red{In the following we define a strictly dominated action which will be a useful concept in finding the Nash equilibrium. }

In the game $\Gamma$, we can iteratively remove the strictly dominated actions. This process is called the iterated elimination of strictly dominated strategies, defined below.
%
\begin{definition}[Iterated elimination] \label{def:elimination_strict}
Set the initial set of actions $A_i^0 = [0,1]$ for all $i$, and for any $k\in \naturals$ let 
\begin{equation}
	\begin{aligned}
	A_i^k = \{a_i \in &A_i^{k-1} \given \\
	&a_i \text{ is not strictly dominated by any } a_{\ccalN_i} \in A_{\ccalN_i}^{k-1}\}.
	\end{aligned}
\end{equation}
%	
\end{definition}
%
We denote the set of player $i$'s actions that survive the iterated elimination by $A_i^\infty := \bigcap_{k =0}^\infty A_i^k$. If $A_i^\infty$ is a singleton (has a single element) for all $i\in\ccalN$, then the game is dominance solvable, and has a unique Nash equilibrium given by the action profile that survives the iterated elimination process. 
%
\subsection{Convergence}
%

%\section{Finite time Nash equilibrium learning}
%We define the rational action in the stage game by the Nash equilibrium solution concept. A Nash equilibrium (NE) action profile $a^{NE} \in [0,1]^n$ is such that no individual has a preferable deviation from its action, that is, for a given state $s$,
%%
%\begin{align} \label{Nash_definition}
%u_i(a_i^{NE}, a_{\ccalN_i^C}^{NE}, s_i, s_{\ccalN_i^C}) \geq  u_i(a_i, a_{\ccalN_i^C}^{NE}, s_i, s_{\ccalN_i^C}) \quad a_i \in [0,1],  \forall i \in \ccalN
%\end{align}
%%
%where $a_{\ccalN_i^C}^{NE} := \{a_{j}^{NE}: j\in \ccalN_i^C \}$.
%%
%In other words, the individuals respond to the NE actions of other individuals to maximize their payoffs. For a given state $s_i, s_{\ccalN_i^C}$ and neighbor action profile $a_{\ccalN_i^C}$ we have the best response of individual $i$ as follows,
%%
%\begin{align}
%BR_i(a_{\ccalN_i^C}, s_i, s_{\ccalN_i^C}) &:= \argmax_{a_i \in [0,1]} u_i(a_i, a_{\ccalN_i^C}, s_{\ccalN_i^C})) \label{best_response} \\
%& = \bbone\left({1} > \beta c_0 (1-s_i) \sum_{j\in \ccalN_i^C} a_j s_j + {\beta c_1 s_i \sum_{j\in\ccalN_i^C} a_j (1-s_j)}\right) \label{best_response_specific}
%\end{align}
%%
%where $\bbone(\cdot)$ is an indicator function. Since the payoffs are linear in self-actions, the actions that maximize the payoffs are in the extremes -- $a_i =1$ or $a_i = 0$ -- depending on the states and actions of their neighbors. 
%We can equivalently represent the NE definition in \eqref{Nash_definition} by using the best response definition,  
%%
%\begin{align} \label{NE_best_response}
%a_i^{NE} = BR_i(a_{\ccalN_i^C}^{NE}, s_i, s_{\ccalN_i^C}) \quad \forall i\in \ccalN.
%\end{align}
%%
%In the following we define a strictly dominated action which will be a useful concept in finding the Nash equilibrium. 
%%
%\begin{definition}[Strictly dominated action] \label{strictly_dominated_definition}
%An action $a_i \in [0,1]$ is strictly dominated if and only if there exists an action $a_i' \in [0,1]$ such that 
%\begin{equation}\label{eq:strictly_dominated_definition}
%u_i(a_i', a_{\ccalN_i^C}, s_i, s_{\ccalN_i^C}) >  u_i(a_i, a_{\ccalN_i^C}, s_i, s_{\ccalN_i^C}) \quad \forall a_{\ccalN_i^C}
%\end{equation}
%\end{definition}
%%
%If an action $a_i$ is strictly dominated then there exists a more preferable action $a_i'$ for any circumstance. It is clear that if an action is strictly dominated then it cannot be a rational action from \eqref{NE_best_response}. In a game we can iteratively remove the strictly dominated actions, this process is called the iterated elimination of strictly dominated strategies and is defined below.
%%
%\begin{definition}[Iterated elimination of strictly dominated actions] \label{def:elimination_strict}
%Set the initial set of actions $A_i^0 = [0,1]$ for all $i$, and for any $k\in \naturals$ set 
%\begin{equation}
%A_i^k = \{a_i \in A_i^{k-1} \given a_i \text{ is not strictly dominated given any } a_{\ccalN_i^C} \in A_{\ccalN_i^C}^{k-1}\}
%\end{equation}
%\end{definition}
%%
%We denote the set of actions of individual $i$ that survive the iterated elimination by $A_i^\infty := \bigcap_{k =0}^\infty A_i^k$. When $A_i^\infty$ has a single element, we say $A_i^\infty$ is a singleton. Inspired by the process above, we propose the following local algorithm. 

%\begin{definition}[Local algorithm] \label{local_algorithm}
%Given state $s \in \{0,1\}^n$. Initially set $a_{i,0} = \epsilon$ where $1>\epsilon>0$.  At each iteration $k \in \naturals$, if $a_{i, k-1} \in \{0,1\}$, set $a_{i,k} =a_{i, k-1}$. Otherwise, observe neighbors actions $a_{\ccalN_i^C, k-1}$. If $a_{j, k-1} = a_{j, k-2} =\dots = a_{j, k-n}$ for all $j \in \ccalN_i^C$ when $k \geq n$ then select $a_{i, k} = 1$ if $s_i =0$ or $a_{i, k} = 0$ if $s_i =1$. Otherwise, update $a_{i, k}$ as follows
%%For all $j \in \ccalN_i^C$ define $a'_j = a_{j, k-1}$ if $a_{j, k-1} \in \{0,1\}$, otherwise $a'_j = 1$ when $k$ is odd and $a'_j = 0$ when $k$ is even. Then for $k$ odd, 
%%
%\begin{align} \label{worst_case_good_response_2}
%a_{i,k} = 1 \quad\text{ if } 1 > \beta (c_0 (1-s_i) \sum_{j\in \ccalN_i^C} \left\lceil a_{j,k-1} \right\rceil s_j +  c_1 s_i \sum_{j\in\ccalN_i^C} \left\lceil a_{j,k-1} \right\rceil (1-s_j)),
%\end{align}
%%
%%
%\begin{align} \label{best_case_bad_response_2}
%a_{i,k} = 0 \quad\text{ if } 1 < \beta (c_0 (1-s_i) \sum_{j\in \ccalN_i^C} \lfloor a_{j,k-1} \rfloor s_j + c_1 s_i \sum_{j\in\ccalN_i^C} \lfloor a_{j,k-1} \rfloor(1-s_j))
%\end{align}
%%
%where $\lceil \cdot \rceil$ is the ceil function and $\lfloor \cdot \rfloor$ is the floor function. Otherwise, select $a_{i,k} = \epsilon$. Share $a_{i,k}$ with $j \in \ccalN_i^C$. If $k<2n$, advance the iteration number $k = k+1$.
%\end{definition}

%
%The algorithm above is local, only relies on observing actions of one's neighbors in the network. The update in \eqref{worst_case_good_response} is a \emph{socialize} response to a worst case scenario where besides neighbors that have actions $a_{j,k-1} = 0$, every $j \in \ccalN_i^C$ is considered to be socializing with interaction level 1. Even in this worst possible scenario, if the socializing constant $1$ is larger than the right hand side of the condition in \eqref{worst_case_good_response} then individual $i$ selects to socialize fully. In contrast, the update in \eqref{best_case_bad_response} is a \emph{do not socialize} response to a best case scenario where besides neighbors that announce to socialize fully $a_{j,k-1} = 1$, every $j \in \ccalN_i^C$ is considered to be isolated off from the network. Even in this best possible scenario, if the socializing constant $1$ is smaller than the right hand side of the condition in \eqref{best_case_bad_response} then individual $i$ selects to isolate itself by selecting $a_{i,k} = 0$. If none of the two conditions in \eqref{worst_case_good_response} and \eqref{best_case_bad_response} is satisfied, then the individual makes a provisional social interaction decision of $1>\epsilon >0$. We exemplify this algorithm on a simple  network in an illustration -- see Figure \ref{fig:algorithm_example}. 

The following theorem states that Algorithm \ref{local_alg} eliminates all strictly dominated actions in finite number of steps.

%\begin{theorem} \label{local_algorithm_convergence}
%Algorithm \ref{local_alg} converges in at most $n$ iterations, that is, no player changes its action after the $n$th update. At the end of $n$ iterations, if all players are decided, i.e., $a_{i}^n = \{0,1\}$ for all $i\in\ccalN$, then all the other actions $\ccalA_i \setminus a_{i}^n$ are strictly dominated and the resultant action profile is a Nash equilibrium. Otherwise, if a player $i \in \ccalN$ is undecided, i.e., $a_{i}^n = \epsilon$, then there does not exist $a_i \in \ccalA_i$ that can be strictly dominated. 
%\end{theorem}
\begin{theorem} \label{local_algorithm_convergence}
Assume all players are undecided, i.e., $a_{i}^0 = \epsilon$ for $i\in\ccalN$. Algorithm \ref{local_alg} converges in at most $n$ iterations, that is, no player changes its action after the $n$th update. If all players are decided, i.e., $a_{i}^n = \{0,1\}$ for all $i\in\ccalN$, the resultant action profile $a^n$ is a Nash equilibrium. Otherwise, if a player $i \in \ccalN$ is undecided, then there does not exist $a_i \in \ccalA_i$ that can be strictly dominated. 
\end{theorem}

%
%
%if all players are decided, i.e., $a_{i,n} = \{0,1\}$, then the resulting action profile $a \in \ccalA$ is the unique Nash equilibrium. 
%
%In Algorithm \ref{local_alg}, no updates are possible after
%
%if all players are decidd
%
% converges to a pure Nash equilibrium of the game with payoffs given by  \eqref{utility} in $n$ steps. 
%

The proof (see Appendix) relies on showing that Algorithm \ref{local_algorithm_convergence} is a decentralized version of the iterated elimination of strictly dominated actions as given by Definition \ref{def:elimination_strict}. The intuition for $n$ step convergence is that at each step at least one player needs to eliminate its action using \eqref{worst_case_good_response} or \eqref{best_case_bad_response}. If no player updates at a time step, the players stop updating because no new eliminations are triggered. Therefore, there could  at most be $n$ iterations to rule out $n$ players one player at a time.




